Unifying Large Language Models and Knowledge Graphs: A Roadmap

Large language models (LLMs), such as ChatGPT and GPT4, are making new waves in the field of natural language processing and artificial intelligence, due to their emergent ability and generalizability. However, LLMs are black-box models, which often fall short of capturing and accessing factual knowledge. In contrast, Knowledge Graphs (KGs), Wikipedia and Huapu for example, are structured knowledge models that explicitly store rich factual knowledge. KGs can enhance LLMs by providing external knowledge for inference and interpretability. Meanwhile, KGs are difficult to construct and evolving by nature, which challenges the existing methods in KGs to generate new facts and represent unseen knowledge. Therefore, it is complementary to unify LLMs and KGs together and simultaneously leverage their advantages. In this article, we present a forward-looking roadmap for the unification of LLMs and KGs. Our roadmap consists of three general frameworks, namely, 1) KG-enhanced LLMs, which incorporate KGs during the pre-training and inference phases of LLMs, or for the purpose of enhancing understanding of the knowledge learned by LLMs; 2) LLM-augmented KGs, that leverage LLMs for different KG tasks such as embedding, completion, construction, graph-to-text generation, and question answering; and 3) Synergized LLMs + KGs, in which LLMs and KGs play equal roles and work in a mutually beneficial way to enhance both LLMs and KGs for bidirectional reasoning driven by both data and knowledge. We review and summarize existing efforts within these three frameworks in our roadmap and pinpoint their future research directions.

==> bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/shirui-bio.jpg}}]{Shirui Pan} received a Ph.D. in computer science from the University of Technology Sydney (UTS), Ultimo, NSW, Australia. He is a Professor with the School of Information and Communication Technology, Griffith University, Australia.
    % Senior Lecturer with the Faculty of Information Technology, Monash University, Australia.
    Prior to this, he was a Senior Lecturer with the Faculty of IT at Monash University.
    His research interests include data mining and machine learning. To date, Dr Pan has published over 100 research papers in top-tier journals and conferences, including TPAMI, TKDE, TNNLS, ICML, NeurIPS, and KDD. His research has attracted over 20,000 citations. His research received the 2024 CIS IEEE TNNLS Oustanding Paper Award and the 2020 IEEE ICDM Best Student Paper Award. He is recognised as one of the AI 2000 AAAI/IJCAI Most Influential Scholars in Australia (2021). He is an ARC Future Fellow and a Fellow of Queensland Academy of Arts and Sciences (FQA).
\end{IEEEbiography}

% \vspace{-1.5cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/linhaoluo.jpg}}]{Linhao Luo} received the bachelor degree from the Harbin Institute of Technology, Shenzhen in 2021. He is now a PhD student in the faculty of information and technology at Monash University. His research interests include machine learning, data mining, and graph neural networks.
\end{IEEEbiography}

% \vspace{-1.5cm}
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/yufeiwang.jpg}}]{Yufei Wang} is a research associate at Monash University, Australia. He obtained his PhD and research-based master degree from Macquarie University, under supervision of Prof. Mark Johnson in 2023 and 2019, respectively. He earned his Bachelor degree jointly from University of Queensland and Sun-Yat Sen University in 2016. His research interests include large language models, natural language processing and controllable text generation.
\end{IEEEbiography}

% \vspace{-1.5cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/JiapuWang.pdf}}]{Jiapu Wang} is currently a Ph.D student in the Beijing Municipal Key Laboratory of Multimedia and Intelligent Software Technology, Beijing University of Technology, Beijing. His research interests include knowledge graph completion, computer vision and pattern recognition.
\end{IEEEbiography}
% \vspace{-1.5cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/chenchen.jpg}}]{Chen Chen} received his Bachelor degree from the University of Science and technology Beijing, China in 2012. He completed his Master of Computer Science from the University of New South Wales, Australia in 2018 and then continued his study to Doctor of Philosophy (PhD) in Nanyang technological University, Singapore. His research interests lie in the area of Natural Language Processing, Knowledge Graphs and Large Language Model.
\end{IEEEbiography}
\vspace{-1.5cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/xindongwu.JPG}}]{Xindong Wu} is Director and Professor of the Key Laboratory of Knowledge Engineering with Big Data (the Ministry of Education of China), Hefei University of Technology, China. He is also a Senior Research Scientist at Zhejiang Lab, China. His research interests include big data analytics, data mining and knowledge engineering. He received his Bachelor's and Master's degrees in Computer Science from the Hefei University of Technology, China, and his Ph.D. degree in Artificial Intelligence from the University of Edinburgh, Britain. He is a Foreign Member of the Russian Academy of Engineering, and a Fellow of IEEE and the AAAS (American Association for the Advancement of Science).

Dr. Wu is the Steering Committee Chair of the IEEE International Conference on Data Mining (ICDM), and the Editor in-Chief of Knowledge and Information Systems (KAIS, by Springer). He was the Editor-in-Chief of the IEEE Transactions on Knowledge and Data Engineering (TKDE) between 2005 and 2008 and Co-Editor-in-Chief of the ACM Transactions on Knowledge Discovery from Data Engineering between 2017 and 2020. He served as a program committee chair/co-chair for ICDM 2003 (the 3rd IEEE International Conference on Data Mining), KDD 2007 (the 13th ACM SIGKDD International Conference on Knowledge Discovery and Data Mining), CIKM 2010 (the 19th ACM Conference on Information and Knowledge Management), and ICBK 2017 (the 8th IEEE International Conference on Big Knowledge). One of his completed projects is Knowledge Engineering With Big Data (BigKE), which was a 54-month, 45-million RMB, 15-institution national grand project, as described in detail at https://ieeexplore.ieee.org/abstract/document/7948800

\end{IEEEbiography}

==> sections/LLM_for_KG_Full.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
    \centering
    \caption{Summary of representative LLM-augmented KG methods.}
    \label{tab:summary_of_LLMs_for_kgs}
    %\resizebox{\columnwidth}{!}{%
    \begin{threeparttable}[b]
        \begin{tabular}{@{}l|llll@{}}
            \toprule
            Task                                           & Method                                               & Year & LLM &Technique                            \\ \midrule
            \multirow{8}{*}{LLM-augmented KG embedding}          & Pretrain-KGE \cite{zhang2020pretrain}                & 2020 & \textbf{E} & LLMs as Text Encoders                \\
                                                            & KEPLER \cite{wang-etal-2021-kepler}                         & 2020 & \textbf{E} & LLMs as Text Encoders                \\
                                                            & Nayyeri et al. \cite{nayyeri2022integrating}         & 2022 & \textbf{E} & LLMs as Text Encoders                \\
                                                            & Huang et al. \cite{huang2022endowing}                & 2022 & \textbf{E} & LLMs as Text Encoders                \\
                                                            & CoDEx \cite{alam2022language}                        & 2022 & \textbf{E} & LLMs as Text Encoders                \\ \cmidrule(l){2-5}
                                                            & LMKE \cite{wang2022language}                         & 2022 & \textbf{E} & LLMs for Joint Text and KG Embedding \\
                                                            & kNN-KGE \cite{zhang2022reasoning}                    & 2022 & \textbf{E} & LLMs for Joint Text and KG Embedding \\
                                                            & LambdaKG \cite{lambdakg}                             & 2023 & \textbf{E} + \textbf{D} + \textbf{ED} & LLMs for Joint Text and KG Embedding \\ \midrule
            \multirow{12}{*}{LLM-augmented KG completion}        & KG-BERT~\cite{yao2019kg}                               & 2019 & \textbf{E} & Joint Encoding                       \\
                                                            & MTL-KGC~\cite{MTL-KGC}                               & 2020 & \textbf{E} & Joint Encoding                       \\
                                                            & PKGC~\cite{PKGC}                                     & 2022 & \textbf{E} & Joint Encoding                       \\
                                                            & LASS~\cite{LASS}                                     & 2022 & \textbf{E} & Joint Encoding                       \\ \cmidrule(l){2-5}
                                                            & MEM-KGC~\cite{MEM-KGC}                               & 2021 & \textbf{E} & MLM Encoding                         \\
                                                            & OpenWorld KGC \cite{open-world-KGC}                  & 2023 & \textbf{E} & MLM Encoding                         \\ \cmidrule(l){2-5}
                                                            & StAR~\cite{StAR}                                     & 2021 & \textbf{E} & Separated Encoding                   \\
                                                            & SimKGC~\cite{SimKGC}                                 & 2022 & \textbf{E} & Separated Encoding                   \\
                                                            & LP-BERT \cite{LP-BERT}                               & 2022 & \textbf{E} & Separated Encoding                   \\ \cmidrule(l){2-5}
                                                            & GenKGC~\cite{GenKGC}                                 & 2022 & \textbf{ED} & LLM as decoders                      \\
                                                            & KGT5~\cite{KGT5}                                     & 2022 & \textbf{ED} & LLM as decoders                      \\
                                                            & KG-S2S~\cite{KG-S2S}                                 & 2022 & \textbf{ED} & LLM as decoders                      \\
                                                            & AutoKG~\cite{zhu2023llms} & 2023 & \textbf{D} & LLM as decoders \\
                                                            \midrule
            \multirow{18}{*}{LLM-augmented KG construction}      & ELMO \cite{Elmo} & 2018 & \textbf{E} & Named Entity Recognition \\
            & GenerativeNER \cite{generativeNER} & 2021 & \textbf{ED} & Named Entity Recognition \\
                                                            & LDET \cite{LDET}                                     & 2019 & \textbf{E} & Entity Typing                        \\
                                                            & BOX4Types \cite{BOX4Types}                           & 2021 & \textbf{E} & Entity Typing                        \\
                                                            & ELQ~\cite{ELQ}                                       & 2020 & \textbf{E} & Entity Linking                       \\
                                                            & ReFinED \cite{ReFinED}                                 & 2022 & \textbf{E} & Entity Linking                       \\ \cmidrule(l){2-5}
                                                            & BertCR \cite{CR1}                                    & 2019 & \textbf{E} & CR (Within-document)                 \\
                                                            & Spanbert \cite{SpanBERT}                             & 2020 & \textbf{E} & CR (Within-document)                 \\
                                                            & CDLM \cite{CDLM}                                     & 2021 & \textbf{E} & CR (Cross-document)                  \\
                                                            & CrossCR \cite{crossCR}                               & 2021 & \textbf{E} & CR (Cross-document)                  \\
                                                            & CR-RL \cite{CR-RL}                                   & 2021 & \textbf{E} & CR (Cross-document)                  \\ \cmidrule(l){2-5}
                                                            & SentRE \cite{sent-re1}                               & 2019 & \textbf{E} & RE (Sentence-level)                  \\
                                                            & Curriculum-RE \cite{Curriculum-RE}                   & 2021 & \textbf{E} & RE (Sentence-level)                  \\
                                                            & DREEAM \cite{DREEAM}                                 & 2023 & \textbf{E} & RE (Document-level)                  \\ \cmidrule(l){2-5}
                                                            & Kumar et al. \cite{kumar2020building}                & 2020 & \textbf{E} & End-to-End Construction              \\
                                                            & Guo et al. \cite{guo2021constructing}                & 2021 & \textbf{E} & End-to-End Construction              \\
                                                            & Grapher \cite{melnyk2021grapher}                     & 2021 & \textbf{ED} & End-to-End Construction              \\
                                                            & PiVE \cite{han2023pive}                              & 2023 & \textbf{D} +  \textbf{ED} & End-to-End Construction              \\
            \cmidrule(l){2-5}
                                                            & COMET \cite{bosselut2019comet}                       & 2019 & \textbf{D}  & Distilling KGs from LLMs             \\
                                                            & BertNet \cite{hao2022bertnet}                        & 2022 & \textbf{E} & Distilling KGs from LLMs             \\
                                                            & West et al. \cite{west2022symbolic}                  & 2022 & \textbf{D} & Distilling KGs from LLMs             \\ \midrule
            \multirow{6}{*}{LLM-augmented KG-to-text Generation} & Ribeiro et al \cite{ribeiro-etal-2021-investigating} & 2021 & \textbf{ED} & Leveraging Knowledge from LLMs       \\                                      
            & JointGT \cite{ke-etal-2021-jointgt}                  & 2021 & \textbf{ED} & Leveraging Knowledge from LLMs       \\
                                                            & FSKG2Text \cite{li-etal-2021-shot-knowledge}         & 2021 & \textbf{D} + \textbf{ED}& Leveraging Knowledge from LLMs       \\
                                                            & GAP \cite{colas-etal-2022-gap}                       & 2022 & \textbf{ED} & Leveraging Knowledge from LLMs       \\ \cmidrule(l){2-5}
                                                            & GenWiki \cite{jin-etal-2020-genwiki}                 & 2020 & - & Constructing KG-text aligned Corpus  \\
                                                            & KGPT \cite{chen-etal-2020-kgpt}                      & 2020 & \textbf{ED} & Constructing KG-text aligned Corpus  \\ \midrule
            \multirow{10}{*}{LLM-augmented KGQA}                                                                             & Lukovnikov et al. \cite{lukovnikov2019pretrained}    & 2019 & \textbf{E}  & Entity/Relation Extractor            \\
            & Luo et al. \cite{luo2020bert}                        & 2020 & \textbf{E} & Entity/Relation Extractor            \\
                                                            & QA-GNN \cite{yasunaga-etal-2021-qa}                  & 2021 & \textbf{E} & Entity/Relation Extractor            \\
                                                            & Nan et al. \cite{hu2023empirical}                    & 2023 & \textbf{E} + \textbf{D} + \textbf{ED} & Entity/Relation Extractor            \\ \cmidrule(l){2-5}
                                                            & DEKCOR \cite{xu2021fusing}                           & 2021 & \textbf{E} & Answer Reasoner                      \\
                                                            & DRLK \cite{zhang2022drlk}                            & 2022 & \textbf{E} & Answer Reasoner                      \\
                                                            & OreoLM \cite{hu2022empowering}                       & 2022 & \textbf{E} & Answer Reasoner                      \\
                                                            & GreaseLM \cite{zhang2022greaselm}                    & 2022 & \textbf{E} & Answer Reasoner                      \\
                                                            & ReLMKG \cite{cao2022relmkg}                          & 2022 & \textbf{E} & Answer Reasoner                      \\
                                                            & UniKGQA \cite{jiang2023unikgqa}                      & 2023 & \textbf{E} & Answer Reasoner                      \\ \bottomrule
        \end{tabular}%
        \begin{tablenotes}
            \item \textbf{E}: Encoder-only LLMs, \textbf{D}: Decoder-only LLMs, \textbf{ED}: Encoder-decoder LLMs.
          \end{tablenotes}
         \end{threeparttable}
    %}
\end{table*}

\section{LLM-augmented KGs}\label{sec:LLM_for_KG}
Knowledge graphs are famous for representing knowledge in a structural manner. They have been applied in many downstream tasks such as question answering, recommendation, and web search. However, the conventional KGs are often incomplete and existing methods often lack considering textual information. To address these issues, recent research has explored integrating LLMs to augment KGs to consider the textual information and improve the performance in downstream tasks. In this section, we will introduce the recent research on LLM-augmented KGs. Representative works are summarized in Table \ref{tab:summary_of_LLMs_for_kgs}. We will introduce the methods that integrate LLMs for KG embedding, KG completion, KG construction, KG-to-text generation, and KG question answering, respectively.


\subsection{LLM-augmented KG Embedding}
Knowledge graph embedding (KGE) aims to map each entity and relation into a low-dimensional vector (embedding) space. These embeddings contain both semantic and structural information of KGs, which can be utilized for various tasks such as question answering \cite{huang2019knowledge}, reasoning \cite{lin-etal-2019-kagnet}, and recommendation \cite{wang2018dkn}. Conventional knowledge graph embedding methods mainly rely on the structural information of KGs to optimize a scoring function defined on embeddings (e.g., TransE \cite{bordes2013translating}, and DisMult \cite{yang2015embedding}). However, these approaches often fall short in representing unseen entities and long-tailed relations due to their limited structural connectivity \cite{xiong2018one,wang2019logic}. To address this issue, as shown in Fig. \ref{fig:LLM_for_KGE}, recent research adopt LLMs to enrich representations of KGs by encoding the textual descriptions of entities and relations \cite{zhang2020pretrain,wang-etal-2021-kepler}.

\subsubsection{LLMs as Text Encoders}
Pretrain-KGE \cite{zhang2020pretrain} is a representative method that follows the framework shown in Fig. \ref{fig:LLM_for_KGE}. Given a triple $(h,r,t)$ from KGs, it firsts uses a LLM encoder to encode the textual descriptions of entities $h$, $t$, and relations $r$ into representations as
\begin{gather}
    e_h = \text{LLM}(\text{Text}_h),
    e_t = \text{LLM}(\text{Text}_t),
    e_r = \text{LLM}(\text{Text}_r),
\end{gather}
where $e_h,e_r,$ and $e_t$ denotes the initial embeddings of entities $h$, $t$, and relations $r$, respectively. Pretrain-KGE uses the BERT as the LLM encoder in experiments. Then, the initial embeddings are fed into a KGE model to generate the final embeddings $v_h,v_r$, and $v_t$. During the KGE training phase, they optimize the KGE model by following the standard KGE loss function as
\begin{equation}
    \mathcal{L} = [\gamma + f(v_h,v_r,v_t)-f(v'_h,v'_r,v'_t)],
\end{equation}
where $f$ is the KGE scoring function, $\gamma$ is a margin hyperparameter, and $v'_h,v'_r$, and $v'_t$ are the negative samples. In this way, the KGE model could learn adequate structure information, while reserving partial knowledge from LLM enabling better knowledge graph embedding. KEPLER \cite{wang-etal-2021-kepler} offers a unified model for knowledge embedding and pre-trained language representation. This model not only generates effective text-enhanced knowledge embedding using powerful LLMs but also seamlessly integrates factual knowledge into LLMs. Nayyeri et al. \cite{nayyeri2022integrating} use LLMs to generate the world-level, sentence-level, and document-level representations. They are integrated with graph structure embeddings into a unified vector by Dihedron and Quaternion representations of 4D hypercomplex numbers. Huang et al. \cite{huang2022endowing} combine LLMs with other vision and graph encoders to learn multi-modal knowledge graph embedding that enhances the performance of downstream tasks. CoDEx \cite{alam2022language} presents a novel loss function empowered by LLMs that guides the KGE models in measuring the likelihood of triples by considering the textual information. The proposed loss function is agnostic to model structure that can be incorporated with any KGE model.

\begin{figure}[]
    \centering
    \includegraphics[width=0.7\columnwidth]{figs/LLM_for_KGE.pdf}
    \caption{LLMs as text encoder for knowledge graph embedding (KGE).}
    \label{fig:LLM_for_KGE}
\end{figure}

\subsubsection{LLMs for Joint Text and KG Embedding}
Instead of using KGE model to consider graph structure, another line of methods directly employs LLMs to incorporate both the graph structure and textual information into the embedding space simultaneously. As shown in Fig. \ref{fig:LLM_for_KGE_2}, $k$NN-KGE \cite{zhang2022reasoning} treats the entities and relations as special tokens in the LLM. During training, it transfers each triple $(h,r,t)$ and corresponding text descriptions into a sentence $x$ as
\begin{equation}
    x = \texttt{[CLS]} \ h \ \ \text{Text}_h \texttt{[SEP]} \ r  \ \texttt{[SEP]} \ \texttt{[MASK]} \ \ \text{Text}_t \texttt{[SEP]},
\end{equation}
where the tailed entities are replaced by \texttt{[MASK]}. The sentence is fed into a LLM, which then finetunes the model to predict the masked entity, formulated as
\begin{equation}
    P_{LLM}(t|h,r) = P(\texttt{[MASK]=t}|x, \Theta), \label{eq:LLM_kge_masking}
\end{equation}
where $\Theta$ denotes the parameters of the LLM. The LLM is optimized to maximize the probability of the correct entity $t$. After training, the corresponding token representations in LLMs are used as embeddings for entities and relations. Similarly, LMKE \cite{wang2022language} proposes a contrastive learning method to improve the learning of embeddings generated by LLMs for KGE. Meanwhile, to better capture graph structure, LambdaKG \cite{lambdakg} samples 1-hop neighbor entities and concatenates their tokens with the triple as a sentence feeding into LLMs.

\begin{figure}[]
    \centering
    \includegraphics[width=0.8\columnwidth]{figs/LLM_for_KGE_2.pdf}
    \caption{LLMs for joint text and knowledge graph embedding.}
    \label{fig:LLM_for_KGE_2}
\end{figure}

\subsection{LLM-augmented KG Completion}

Knowledge Graph Completion (KGC) refers to the task of inferring missing facts in a given knowledge graph. Similar to KGE, conventional KGC methods mainly focused on the structure of the KG, without considering the extensive textual information. However, the recent integration of LLMs enables KGC methods to encode text or generate facts for better KGC performance. These methods fall into two distinct categories based on their utilization styles: \emph{1) LLM as Encoders (PaE)}, and \emph{2) LLM as Generators (PaG)}.
\subsubsection{LLM as Encoders (PaE).} As shown in Fig. \ref{fig:PaE} (a), (b), and (c), this line of work first uses encoder-only LLMs to encode textual information as well as KG facts. Then, they predict the plausibility of the triples or masked entities by feeding the encoded representation into a prediction head, which could be a simple MLP or conventional KG score function (e.g., TransE \cite{bordes2013translating} and TransR \cite{lin2015learning}).

\textbf{Joint Encoding.}
Since the encoder-only LLMs (e.g., Bert \cite{devlin2018bert}) are well at encoding text sequences, KG-BERT~\cite{yao2019kg} represents a triple $(h, r, t)$ as a text sequence and encodes it with LLM Fig.~\ref{fig:PaE}(a).
\begin{equation}
    x = \texttt{[CLS]} \ \text{Text}_h \ \texttt{[SEP]} \ \text{Text}_r \ \texttt{[SEP]} \ \text{Text}_t \ \texttt{[SEP]},
\end{equation}
% where [CLS] and [SEP] are reserved tokens and $h^{i}, r^{i}$ and $t^{i}$ denote text tokens of $h, r, t$ respectively.
The final hidden state of the $\texttt{[CLS]}$ token is fed into a classifier to predict the possibility of the triple, formulated as
\begin{equation}
    s = \sigma(\text{MLP}(e_{\texttt{[CLS]}})),
\end{equation}
where $\sigma(\cdot)$ denotes the sigmoid function and $e_{\texttt{[CLS]}}$ denotes the representation encoded by LLMs.
To improve the efficacy of KG-BERT, MTL-KGC~\cite{MTL-KGC} proposed a Multi-Task Learning for the KGC framework which incorporates additional auxiliary tasks into the model's training, i.e. prediction (RP) and relevance ranking (RR). PKGC~\cite{PKGC} assesses the validity of a triplet $(h, r, t)$ by transforming the triple and its supporting information into natural language sentences with pre-defined templates. These sentences are then processed by LLMs for binary classification. The supporting information of the triplet is derived from the attributes of $h$ and $t$ with a verbalizing function. For instance, if the triple is \textit{(Lebron James, member of sports team, Lakers)}, the information regarding Lebron James is verbalized as "Lebron James: American basketball player". LASS~\cite{LASS} observes that language semantics and graph structures are equally vital to KGC. As a result, LASS is proposed to jointly learn two types of embeddings: semantic embedding and structure embedding. In this method, the full text of a triple is forwarded to the LLM, and the mean pooling of the corresponding LLM outputs for $h$, $r$, and $t$ are separately calculated. These embeddings are then passed to a graph-based method, i.e. TransE, to reconstruct the KG structures.

\begin{figure}[]
    \centering
    \includegraphics[width=.7\columnwidth]{figs/PaE.pdf}
    \caption{The general framework of adopting LLMs as encoders (PaE) for KG Completion.}
    \label{fig:PaE}
\end{figure}

\textbf{MLM Encoding.} Instead of encoding the full text of a triple, many works introduce the concept of Masked Language Model (MLM) to encode KG text (Fig.~\ref{fig:PaE}(b)). MEM-KGC~\cite{MEM-KGC} uses Masked Entity Model (MEM) classification mechanism to predict the masked entities of the triple. The input text is in the form of
\begin{equation}
    x = \texttt{[CLS]} \ \text{Text}_h \ \texttt{[SEP]} \ \text{Text}_r  \ \texttt{[SEP]} \ \texttt{[MASK]} \ \texttt{[SEP]},\label{eq:mlm_masking}
\end{equation}
Similar to Eq. \ref{eq:LLM_kge_masking}, it tries to maximize the probability that the masked entity is the correct entity $t$.
Additionally, to enable the model to learn unseen entities, MEM-KGC integrates multitask learning for entities and super-class prediction based on the text description of entities:
\begin{equation}
    x = \texttt{[CLS]} \ \texttt{[MASK]} \ \texttt{[SEP]} \ \text{Text}_h \ \texttt{[SEP]}. \label{eq:edp}
\end{equation}
OpenWorld KGC \cite{open-world-KGC} expands the MEM-KGC model to address the challenges of open-world KGC with a pipeline framework, where two sequential MLM-based modules are defined: Entity Description Prediction (EDP), an auxiliary module that predicts a corresponding entity with a given textual description; Incomplete Triple Prediction (ITP), the target module that predicts a plausible entity for a given incomplete triple $(h, r, ?)$. EDP first encodes the triple with Eq.~\ref{eq:edp} and generates the final hidden state, which is then forwarded into ITP as an embedding of the head entity in Eq.~\ref{eq:mlm_masking} to predict target entities.

\textbf{Separated Encoding.} As shown in Fig.~\ref{fig:PaE}(c), these methods involve partitioning a triple $(h, r, t)$ into two distinct parts, i.e. $(h, r)$ and $t$, which can be expressed as
\begin{align}
    x_{(h,r)} & = \texttt{[CLS]} \ \text{Text}_h \ \texttt{[SEP]} \ \text{Text}_r \ \texttt{[SEP]}, \\
    x_{t}     & = \texttt{[CLS]} \ \text{Text}_t \ \texttt{[SEP]}.
\end{align}
Then the two parts are encoded separately by LLMs, and the final hidden states of the $\texttt{[CLS]}$ tokens are used as the representations of $(h, r)$ and $t$, respectively. The representations are then fed into a scoring function to predict the possibility of the triple, formulated as
\begin{equation}
    s = f_{score} (e_{(h,r)}, e_{t}),
\end{equation}
where $f_{score}$ denotes the score function like TransE.

StAR~\cite{StAR} applies Siamese-style textual encoders on their text, encoding them into separate contextualized representations. To avoid the combinatorial explosion of textual encoding approaches, e.g., KG-BERT, StAR employs a scoring module that involves both deterministic classifier and spatial measurement for representation and structure learning respectively, which also enhances structured knowledge by exploring the spatial characteristics. SimKGC~\cite{SimKGC} is another instance of leveraging a Siamese textual encoder to encode textual representations. Following the encoding process, SimKGC applies contrastive learning techniques to these representations. This process involves computing the similarity between the encoded representations of a given triple and its positive and negative samples. In particular, the similarity between the encoded representation of the triple and the positive sample is maximized, while the similarity between the encoded representation of the triple and the negative sample is minimized. This enables SimKGC to learn a representation space that separates plausible and implausible triples. To avoid overfitting textural information, CSPromp-KG~\cite{CSProm-KG} employs parameter-efficient prompt learning for KGC.

LP-BERT \cite{LP-BERT} is a hybrid KGC method that combines both MLM Encoding and Separated Encoding. This approach consists of two stages, namely pre-training and fine-tuning. During pre-training, the method utilizes the standard MLM mechanism to pre-train a LLM with KGC data. During the fine-tuning stage, the LLM encodes both parts and is optimized using a contrastive learning strategy (similar to SimKGC~\cite{SimKGC}).


\subsubsection{LLM as Generators (PaG).}

\begin{figure}[]
    \centering
    \includegraphics[width=.8\columnwidth]{figs/PaG.pdf}
    \caption{The general framework of adopting LLMs as decoders (PaG) for KG Completion. The En. and De. denote the encoder and decoder, respectively.}
    \label{fig:PaG}
\end{figure}

Recent works use LLMs as sequence-to-sequence generators in KGC. As presented in Fig.~\ref{fig:PaG} (a) and (b), these approaches involve encoder-decoder or decoder-only LLMs. The LLMs receive a sequence text input of the query triple $(h, r, ?)$, and generate the text of tail entity $t$ directly.

GenKGC~\cite{GenKGC} uses the large language model BART~\cite{lewis2020bart} as the backbone model. Inspired by the in-context learning approach used in GPT-3~\cite{brown2020language}, where the model concatenates relevant samples to learn correct output answers, GenKGC proposes a relation-guided demonstration technique that includes triples with the same relation to facilitating the model's learning process. In addition, during generation, an entity-aware hierarchical decoding method is proposed to reduce the time complexity. KGT5~\cite{KGT5} introduces a novel KGC model that fulfils four key requirements of such models: scalability, quality, versatility, and simplicity. To address these objectives, the proposed model employs a straightforward T5 small architecture. The model is distinct from previous KGC methods, in which it is randomly initialized rather than using pre-trained models. KG-S2S~\cite{KG-S2S} is a comprehensive framework that can be applied to various types of KGC tasks, including Static KGC, Temporal KGC, and Few-shot KGC. To achieve this objective, KG-S2S reformulates the standard triple KG fact by introducing an additional element, forming a quadruple $(h, r, t, m)$, where $m$ represents the additional "condition" element. Although different KGC tasks may refer to different conditions, they typically have a similar textual format, which enables unification across different KGC tasks. The KG-S2S approach incorporates various techniques such as entity description, soft prompt, and Seq2Seq Dropout to improve the model's performance. In addition, it utilizes constrained decoding to ensure the generated entities are valid. For closed-source LLMs (e.g., ChatGPT and GPT-4), AutoKG adopts prompt engineering to design customized prompts \cite{zhu2023llms}. As shown in Fig. \ref{fig:prompt_kgc}, these prompts contain the task description, few-shot examples, and test input, which instruct LLMs to predict the tail entity for KG completion.





% \subsubsection{Comparison between PaE and PaG}
% % \todo{We can add a decision tree or a table here for choosing between PaE and PaG or illustrate the pros and cons for PaE and PaG.}
% LLMs as Encoders (PaE) applies an additional prediction head on the top of the representation encoded by LLMs. Therefore, the PaE framework is much easier to finetune since we can only optimize the prediction heads and freeze the LLMs. Moreover, the output of the prediction can be easily specified and integrated with existing KGC functions for different KGC tasks. However, during the inference stage, the PaE requires to compute a score for every candidate in KGs, which could be computationally expensive. Besides, they cannot generalize to unseen entities. Furthermore, the PaE requires the representation output of the LLMs, whereas some state-of-the-art LLMs (e.g. GPT-4\footnotemark[1]) are closed sources and do not grant access to the representation output.

% LLMs as Generators (PaG), on the other hand, which does not need the prediction head, can be used without finetuning or access to representations. Therefore, the framework of PaG is suitable for all kinds of LLMs. In addition, PaG directly generates the tail entity, making it efficient in inference without ranking all the candidates and easily generalizing to unseen entities. But, the challenge of PaG is that the generated entities could be diverse and not lie in KGs. What is more, the time of a single inference is longer due to the auto-regressive generation. Last, how to design a powerful prompt that feeds KGs into LLMs is still an open question.
% Consequently, while PaG has demonstrated promising results for KGC tasks, the trade-off between model complexity and computational efficiency must be carefully considered when selecting an appropriate LLM-based KGC framework.

\begin{figure}[]
    \centering
    \includegraphics[width=.7\columnwidth]{figs/prompt_kgc.pdf}
    \caption{The framework of prompt-based PaG for KG Completion.}
    \label{fig:prompt_kgc}
\end{figure}

% One of the key challenges associated with utilizing LLMs as a Generator in KGC is the significant increase in inference time. This is due to the autoregressive nature of the model's entity text generation process, which is notably slower than alternative approaches that use LLMs as encoders. Consequently, while LLMs as generators have demonstrated promising results for KGC tasks, the trade-off between model complexity and computational efficiency must be carefully considered when selecting an appropriate KGC approach.

\subsubsection{Model Analysis}
Justin et al. \cite{KGC_analysis} provide a comprehensive analysis of KGC methods integrated with LLMs. Their research investigates  the quality of LLM embeddings and finds that they are suboptimal for effective entity ranking. In response, they propose several techniques for processing embeddings to improve their suitability for candidate retrieval. The study also compares different model selection dimensions, such as Embedding Extraction, Query Entity Extraction, and Language Model Selection. Lastly, the authors propose a framework that effectively adapts LLM for knowledge graph completion.









\subsection{LLM-augmented KG Construction}

% \begin{figure}[]
%     \centering
%     \includegraphics[width=0.7\columnwidth]{figs/LLM_for_KGConstruction.pdf}
%     \caption{The general framework of applying LLMs for knowledge graph construction.}
%     \label{fig:LLM_for_KGConsturction}
% \end{figure}
Knowledge graph construction involves creating a structured representation of knowledge within a specific domain. This includes identifying entities and their relationships with each other. The process of knowledge graph construction typically involves multiple stages, including \emph{1) entity discovery}, \emph{2) coreference resolution}, and \emph{3) relation extraction}. Fig~\ref{fig: KGConsturction} presents the general framework of applying LLMs for each stage in KG construction. More recent approaches have explored \emph{4) end-to-end knowledge graph construction}, which involves constructing a complete knowledge graph in one step or directly \emph{5) distilling knowledge graphs from LLMs}.

\subsubsection{Entity Discovery}
Entity discovery in KG construction refers to the process of identifying and extracting entities from unstructured data sources, such as text documents, web pages, or social media posts, and incorporating them to construct knowledge graphs.

\textbf{Named Entity Recognition (NER)} involves identifying and tagging named entities in text data with their positions and classifications. The named entities include people, organizations, locations, and other types of entities. The state-of-the-art NER methods usually employ LLMs to leverage their contextual understanding and linguistic knowledge for accurate entity recognition and classification. There are three NER sub-tasks based on the types of NER spans identified, i.e., flat NER, nested NER, and discontinuous NER. \emph{1) Flat NER is to identify non-overlapping named entities from input text.} It is usually conceptualized as a sequence labelling problem where each token in the text is assigned a unique label based on its position in the sequence~\cite{Elmo,devlin2018bert,Larger-Context-Tagging,Ptuning-v2}. \emph{2) Nested NER considers complex scenarios which allow a token to belong to multiple entities.} The span-based method~\cite{NER-as-DP,DiscontinuousNER,Span-based-NER1,Span-based-NER2,Span-based-NER3} is a popular branch of nested NER which involves enumerating all candidate spans and classifying them into entity types (including a non-entity type). Parsing-based methods~\cite{parserNER1,parserNER2,parserNER3} reveal similarities between nested NER and constituency parsing tasks (predicting nested and non-overlapping spans), and propose to integrate the insights of constituency parsing into nested NER.
% Object-detection-based methods~\cite{OjbDetNER1,OjbDetNER2} leverage the ideas and techniques of object detection tasks in computer vision (CV) to predict ``nested structures'' in nested NER. %https://aclanthology.org/2022.acl-long.428.pdf
\emph{3) Discontinuous NER identifies named entities that may not be contiguous in the text.} To address this challenge, \cite{discontinuousNER1} uses the LLM output to identify entity fragments and determine whether they are overlapped or in succession.

% propose a two-stage approach: In stage 1, the model identifies entity fragments by exploring all possible text spans and in stage 2, relation classification is performed to determine whether given entity fragments overlap or are in succession.  

Unlike the task-specific methods, GenerativeNER \cite{generativeNER} uses a sequence-to-sequence LLM with a pointer mechanism to generate an entity sequence, which is capable of solving all three types of NER sub-tasks.

\begin{figure}[]
    \centering
    \includegraphics[width=\columnwidth]{figs/KGconstruction-v2.pdf}
    \caption{The general framework of LLM-based KG construction.}
    \label{fig: KGConsturction}
\end{figure}

\textbf{Entity Typing (ET)} aims to provide fine-grained and ultra-grained type information for a given entity mentioned in context. These methods usually utilize LLM to encode mentions, context and types. LDET~\cite{LDET} applies pre-trained ELMo embeddings~\cite{Elmo} for word representation and adopts LSTM as its sentence and mention encoders. BOX4Types~\cite{BOX4Types} recognizes the importance of type dependency and uses BERT to represent the hidden vector and each type in a hyperrectangular (box) space. LRN~\cite{LRN} considers extrinsic and intrinsic dependencies between labels. It encodes the context and entity with BERT and employs these output embeddings to conduct deductive and inductive reasoning. MLMET~\cite{MLMET} uses predefined patterns to construct input samples for the BERT MLM and employs [MASK] to predict context-dependent hypernyms of the mention, which can be viewed as type labels. %https://arxiv.org/pdf/2202.06167.pdf
PL~\cite{PL} and DFET~\cite{DFET} utilize prompt learning for entity typing. LITE~\cite{LITE} formulates entity typing as textual inference and uses RoBERTa-large-MNLI as the backbone network. %https://arxiv.org/pdf/2212.09125v1.pdf
% MCCE~\cite{MCCE} performs entity typing in a recall-expand-filter manner, which involves pruning the large type set, generating relevant type candidates and filtering the candidates with their scores to obtain the final prediction.
%https://arxiv.org/pdf/2212.09125v1.pdf
% Neural-PCRF~\cite{Neural-PCRF} utilizes pairwise conditional random field (PCRF) to model the influence between the input and other related type variables.

\textbf{Entity Linking (EL)}, as known as entity disambiguation, involves linking entity mentions appearing in the text to their corresponding entities in a knowledge graph.  \cite{EL1} proposed BERT-based end-to-end EL systems that jointly discover and link entities. ELQ~\cite{ELQ} employs a fast bi-encoder architecture to jointly perform mention detection and linking in one pass for downstream question answering systems. %https://arxiv.org/pdf/2109.12520.pdf
Unlike previous models that frame EL as matching in vector space, GENRE~\cite{GENRE} formulates it as a sequence-to-sequence problem, autoregressively generating a version of the input markup-annotated with the unique identifiers of an entity expressed in natural language. GENRE is extended to its multilingual version mGENRE~\cite{mGENRE}. %https://arxiv.org/pdf/2109.03792v1.pdf
Considering the efficiency challenges of generative EL approaches, \cite{EL2} parallelizes autoregressive linking across all potential mentions and relies on a shallow and efficient decoder. %https://arxiv.org/pdf/2109.03792v1.pdf
ReFinED~\cite{ReFinED} proposes an efficient zero-shot-capable EL approach by taking advantage of fine-grained entity types and entity descriptions which are processed by a LLM-based encoder. %https://arxiv.org/pdf/2207.04108v1.pdf
% EntQA~\cite{EntQA} reorganizes the EL process by performing linking before mention detection.
%https://arxiv.org/pdf/2110.02369v2.pdf
% TempEL~\cite{TempEL} extend the notion of entity linking into dynamically evolving and newly emerging entities. %https://proceedings.neurips.cc/paper_files/paper/2022/file/0c3464f16c854d395b880cf9e7bcaf2f-Paper-Datasets_and_Benchmarks.pdf


\subsubsection{Coreference Resolution (CR)}
Coreference resolution is to find all expressions (i.e., mentions) that refer to the same entity or event in a text.

\textbf{Within-document CR} refers to the CR sub-task where all these mentions are in a single document. Mandar et al. \cite{CR1} initialize LLM-based coreferences resolution by replacing the previous LSTM encoder~\cite{LSTM-CR} with BERT. This work is followed by the introduction of SpanBERT~\cite{SpanBERT} which is pre-trained on BERT architecture with a span-based masked language model (MLM). Inspired by these works, Tuan Manh et al. \cite{CR2} present a strong baseline by incorporating the SpanBERT encoder into a non-LLM approach e2e-coref~\cite{LSTM-CR}. CorefBERT leverages Mention Reference Prediction (MRP) task which masks one or several mentions and requires the model to predict the masked mention’s corresponding referents. CorefQA~\cite{CorefQA} formulates coreference resolution as a question answering task, where contextual queries are generated for each candidate mention and the coreferent spans are extracted from the document using the queries.
% Sopan et al. \cite{CR-type} incorporate external semantic knowledge (i.e., type information) to improve the performance. PAIRWISERL~\cite{PAIRWISERL} utilizes pairwise representation learning to perform both entity and event coreference resolution by concatenating representations of two sentences and their element-wise product. 
Tuan Manh et al. \cite{CR3} introduce a gating mechanism  and a noisy training method to extract information from event mentions using the SpanBERT encoder.
% To identify paraphrase relations between event mentions and avoid propagation errors, EPASE~\cite{EPASE} introduces event-specific paraphrases and argument-aware semantic embeddings to improve the model generalization ability.


In order to reduce the large memory footprint faced by large LLM-based NER models, Yuval et al. \cite{efficientCR1} and Raghuveer el al. \cite{efficientCR2} proposed start-to-end and approximation models, respectively, both utilizing bilinear functions to calculate mention and antecedent scores with reduced reliance on span-level representations.
%To avoid the complexity of span-based coreference resolution models, wl-coref~\cite{wl-coref} prioritizes word-level coreference resolution as a means to reduce computational complexity.


\textbf{Cross-document CR} refers to the sub-task where the mentions refer to the same entity or event might be across multiple documents. CDML \cite{CDLM} proposes a cross document language modeling method which pre-trains a Longformer~\cite{Longformer} encoder on concatenated related documents and employs an MLP for binary classification to determine whether a pair of mentions is coreferent or not. CrossCR \cite{crossCR} utilizes an end-to-end model for cross-document coreference resolution which pre-trained the mention scorer on gold mention spans and uses a pairwise scorer to compare mentions with all spans across all documents. CR-RL \cite{CR-RL} proposes an actor-critic deep reinforcement learning-based coreference resolver for cross-document CR.





%https://sentic.net/survey-on-coreference-resolution.pdf



\subsubsection{Relation Extraction (RE)}
Relation extraction involves identifying semantic relationships between entities mentioned in natural language text. There are two types of relation extraction methods, i.e. sentence-level RE and document-level RE, according to the scope of the text analyzed.

\textbf{Sentence-level RE} focuses on identifying relations between entities within a single sentence. Peng et al. \cite{sent-re1} and TRE~\cite{TRE} introduce LLM to improve the performance of relation extraction models. BERT-MTB~\cite{BERT-MTB} learns relation representations based on BERT by performing the matching-the-blanks task and incorporating designed objectives for relation extraction. Curriculum-RE~\cite{Curriculum-RE} utilizes curriculum learning to improve relation extraction models by gradually increasing the difficulty of the data during training.
% Wenxuan et al.~\cite{sent-re2} identify two issues of previous relation extraction models: 1) inexpressive entity representation, and 2) noisy or ill-defined labels, and introduce a typed entity marker to handle these challenges. 
RECENT~\cite{RECENT} introduces SpanBERT and exploits entity type restriction to reduce the noisy candidate relation types. Jiewen~\cite{sent-re3} extends RECENT by combining both the entity information and the label information into sentence-level embeddings, which enables the embedding to be entity-label aware.
%https://arxiv.org/pdf/2010.11304.pdf
%https://arxiv.org/pdf/2304.04935.pdf

\textbf{Document-level RE (DocRE)} aims to extract relations between entities across multiple sentences within a document. Hong et al. \cite{docRE1} propose a strong baseline for DocRE by replacing the BiLSTM backbone with LLMs. HIN~\cite{HIN} use LLM to encode and aggregate entity representation at different levels, including entity, sentence, and document levels.  GLRE~\cite{GLRE} is a global-to-local network, which uses LLM to encode the document information in terms of entity global and local representations as well as context relation representations. SIRE~\cite{SIRE} uses two LLM-based encoders to extract intra-sentence and inter-sentence relations. LSR~\cite{LSR} and GAIN~\cite{GAIN} propose graph-based approaches which induce graph structures on top of LLM to better extract relations. DocuNet~\cite{DocuNet} formulates DocRE as a semantic segmentation task and introduces a U-Net~\cite{U-net} on the LLM encoder to capture local and global dependencies between entities. ATLOP \cite{ATLOP} focuses on the multi-label problems in DocRE, which could be handled with two techniques, i.e., adaptive thresholding for classifier and localized context pooling for LLM. DREEAM~\cite{DREEAM} further extends and improves ATLOP by incorporating evidence information.
%https://arxiv.org/pdf/2106.03618.pdf
%https://arxiv.org/pdf/2302.08675v1.pdf

% \subsubsection{End-to-End KG Construction}

% Currently, researchers are exploring the use of LLMs for end-to-end KG construction. Kumar et al. \cite{kumar2020building} propose a unified approach to build KGs from raw text, which contains two LLMs powered components. They first finetune a LLM on named entity recognition tasks to make it capable of recognizing entities in raw text. Then, they propose another ``2-model BERT'' for solving the relation extraction task, which contains two BERT-based classifiers. The first classifier learns the relation class whereas the second binary classifier learns the direction of the relations between the two entities. The predicted triples and relations are then used to construct the KG. Guo et al. \cite{guo2021constructing} propose an end-to-end knowledge extraction model based on BERT, which can be applied to construct KGs from Classical Chinese text.
% %During the named entity recognition phase, a BERT-based model is utilized. This model has been pre-trained on Chinese corpus and is used to generate entities, segment, and position embeddings for relation extraction. The generated results are then fed into a BERT encoder to predict relations.
% Grapher \cite{melnyk2021grapher} presents a novel end-to-end multi-stage system. It first utilizes LLMs to generate KG entities, followed by a simple relation construction head, enabling efficient KG construction from the textual description. PiVE \cite{han2023pive} proposes a prompting with an iterative verification framework that utilizes a smaller LLM like T5 to correct the errors in KGs generated by a larger LLM (e.g., ChatGPT). To further explore advanced LLMs, AutoKG design several prompts for different KG construction tasks (e.g., entity typing, entity linking, and relation extraction). Then, it adopts the prompt to perform KG construction using ChatGPT and GPT-4.

\begin{figure}[]
    \centering
    \includegraphics[width=1\columnwidth]{figs/distill_kgs_from_LLMs.pdf}
    \caption{The general framework of distilling KGs from LLMs.}
    \label{fig:distill_kgs}
\end{figure}


\subsubsection{Distilling Knowledge Graphs from LLMs }
LLMs have been shown to implicitly encode massive knowledge \cite{petroni2019language}. As shown in Fig. \ref{fig:distill_kgs}, some research aims to distill knowledge from LLMs to construct KGs.  COMET \cite{bosselut2019comet} proposes a commonsense transformer model that constructs commonsense KGs by using existing tuples as a seed set of knowledge on which to train. Using this seed set, a LLM learns to adapt its learned representations to knowledge generation, and produces novel tuples that are high quality. Experimental results reveal that implicit knowledge from LLMs is transferred to generate explicit knowledge in commonsense KGs. BertNet \cite{hao2022bertnet} proposes a novel framework for automatic KG construction empowered by LLMs. It requires only the minimal definition of relations as inputs and automatically generates diverse prompts, and performs an efficient knowledge search within a given LLM for consistent outputs. The constructed KGs show competitive quality, diversity, and novelty with a richer set of new and complex relations, which cannot be extracted by previous methods. West et al. \cite{west2022symbolic} propose a symbolic knowledge distillation framework that distills symbolic knowledge from LLMs. They first finetune a small student LLM by distilling commonsense facts from a large LLM like GPT-3. Then, the student LLM is utilized to generate commonsense KGs.



\subsection{LLM-augmented KG-to-text Generation}
The goal of Knowledge-graph-to-text (KG-to-text) generation is to generate high-quality texts that accurately and consistently describe the input knowledge graph information~\cite{gardent-etal-2017-webnlg}. KG-to-text generation connects knowledge graphs and texts, significantly improving the applicability of KG in more realistic NLG scenarios, including storytelling~\cite{DBLP:conf/aaai/GuanWH19} and knowledge-grounded dialogue~\cite{DBLP:conf/ijcai/ZhouYHZXZ18}. However, it is challenging and costly to collect large amounts of graph-text parallel data, resulting in insufficient training and poor generation quality. Thus, many research efforts resort to either: \emph{1) leverage knowledge from LLMs} or \emph{2) construct large-scale weakly-supervised KG-text corpus} to solve this issue.

\subsubsection{Leveraging Knowledge from LLMs}
As pioneering research efforts in using LLMs for KG-to-Text generation, Ribeiro et al.~\cite{ribeiro-etal-2021-investigating} and Kale and Rastogi~\cite{kale-rastogi-2020-text} directly fine-tune various LLMs, including BART and T5, with the goal of transferring LLMs knowledge for this task. As shown in Fig. \ref{fig:kg_to_text}, both works simply represent the input graph as a linear traversal and find that such a naive approach successfully outperforms many existing state-of-the-art KG-to-text generation systems. Interestingly, Ribeiro et al.~\cite{ribeiro-etal-2021-investigating} also find that continue pre-training could further improve model performance. However, these methods are unable to \emph{explicitly} incorporate rich graph semantics in KGs. To enhance LLMs with KG structure information, JointGT~\cite{ke-etal-2021-jointgt} proposes to inject KG structure-preserving representations into the Seq2Seq large language models. Given input sub-KGs and corresponding text, JointGT first represents the KG entities and their relations as a sequence of tokens, then concatenate them with the textual tokens which are fed into LLM. After the standard self-attention module, JointGT then uses a pooling layer to obtain the contextual semantic representations of knowledge entities and relations. Finally, these pooled KG representations are then aggregated in another structure-aware self-attention layer. JointGT also deploys additional pre-training objectives, including KG and text reconstruction tasks given masked inputs, to improve the alignment between text and graph information.  Li et al.~\cite{li-etal-2021-shot-knowledge} focus on the few-shot scenario. It first employs a novel breadth-first search (BFS) strategy to better traverse the input KG structure and feed the enhanced linearized graph representations into LLMs for high-quality generated outputs, then aligns the GCN-based and LLM-based KG entity representation. Colas et al.~\cite{colas-etal-2022-gap} first transform the graph into its appropriate representation before linearizing the graph. Next, each KG node is encoded via a global attention mechanism, followed by a graph-aware attention module, ultimately being decoded into a sequence of tokens. Different from these works, KG-BART~\cite{DBLP:conf/aaai/LiuW0PY21} keeps the structure of KGs and leverages the graph attention to aggregate the rich concept semantics in the sub-KG, which enhances the model generalization on unseen concept sets.

\begin{figure}[]
    \centering
    \includegraphics[width=1\columnwidth]{figs/graph_to_text.pdf}
    \caption{The general framework of KG-to-text generation.}
    \label{fig:kg_to_text}
\end{figure}

\subsubsection{Constructing large weakly KG-text aligned Corpus}
Although LLMs have achieved remarkable empirical success, their unsupervised pre-training objectives are not necessarily aligned well with the task of KG-to-text generation, motivating researchers to develop large-scale KG-text aligned corpus. Jin et al.~\cite{jin-etal-2020-genwiki} propose a 1.3M unsupervised KG-to-graph training data from Wikipedia. Specifically, they first detect the entities appearing in the text via hyperlinks and named entity detectors, and then only add text that shares a common set of entities with the corresponding knowledge graph, similar to the idea of distance supervision in the relation extraction task~\cite{mintz-etal-2009-distant}.
They also provide a 1,000+ human annotated KG-to-Text test data to verify the effectiveness of the pre-trained KG-to-Text models. Similarly, Chen et al.~\cite{chen-etal-2020-kgpt} also propose a KG-grounded text corpus collected from the English Wikidump. To ensure the connection between KG and text, they only extract sentences with at least two Wikipedia anchor links. Then, they use the entities from those links to query their surrounding neighbors in WikiData and calculate the lexical overlapping between these neighbors and the original sentences. Finally, only highly overlapped pairs are selected. The authors explore both graph-based and sequence-based encoders and identify their advantages in various different tasks and settings.







\subsection{LLM-augmented KG Question Answering}


Knowledge graph question answering (KGQA) aims to find answers to natural language questions based on the structured facts stored in knowledge graphs \cite{saxena2020improving,feng-etal-2020-scalable}. The inevitable challenge in KGQA is to retrieve related facts and extend the reasoning advantage of KGs to QA. Therefore, recent studies adopt LLMs to bridge the gap between natural language questions and structured knowledge graphs \cite{xu2021fusing,yan2021large,hu2023empirical}. The general framework of applying LLMs for KGQA is illustrated in Fig. \ref{fig:LLM_for_KGQA}, where LLMs can be used as 1) entity/relation extractors, and 2) answer reasoners.

\subsubsection{LLMs as Entity/relation Extractors}
Entity/relation extractors are designed to identify entities and relationships mentioned in natural language questions and retrieve related facts in KGs. Given the proficiency in language comprehension, LLMs can be effectively utilized for this purpose. Lukovnikov et al. \cite{lukovnikov2019pretrained} are the first to utilize LLMs as classifiers for relation prediction, resulting in a notable improvement in performance compared to shallow neural networks. Nan et al. \cite{hu2023empirical} introduce two LLM-based KGQA frameworks that adopt LLMs to detect mentioned entities and relations. Then, they query the answer in KGs using the extracted entity-relation pairs. QA-GNN \cite{yasunaga-etal-2021-qa} uses LLMs to encode the question and candidate answer pairs, which are adopted to estimate the importance of relative KG entities. The entities are retrieved to form a subgraph, where an answer reasoning is conducted by a graph neural network.
Luo et al. \cite{luo2020bert} use LLMs to calculate the similarities between relations and questions to retrieve related facts, formulated as
\begin{equation}
    s(r,q) = \text{LLM}(r)^\top \text{LLM}(q),\label{eq:relation_sim}
\end{equation}
where $q$ denotes the question, $r$ denotes the relation, and $\text{LLM}(\cdot)$ would generate representation for $q$ and $r$, respectively. Furthermore, Zhang et al. \cite{zhang2022subgraph} propose a LLM-based path retriever to retrieve question-related relations hop-by-hop and construct several paths. The probability of each path can be calculated as
\begin{equation}
    P(p|q) = \prod_{t=1}^{|p|} s(r_t,q),\label{eq:path_prob}
\end{equation}
where $p$ denotes the path, and $r_t$ denotes the relation at the $t$-th hop of $p$. The retrieved relations and paths can be used as context knowledge to improve the performance of answer reasoners as
\begin{equation}
    P(a|q) = \sum_{p\in \mathcal{P}} P(a|p)P(p|q),
\end{equation}
where $\mathcal{P}$ denotes retrieved paths and $a$ denotes the answer.

\begin{figure}[]
    \centering
    \includegraphics[width=.8\columnwidth]{figs/LLM_for_KGQA.pdf}
    \caption{The general framework of applying LLMs for knowledge graph question answering (KGQA).}
    \label{fig:LLM_for_KGQA}
\end{figure}

\subsubsection{LLMs as Answer Reasoners}
Answer reasoners are designed to reason over the retrieved facts and generate answers. LLMs can be used as answer reasoners to generate answers directly. For example, as shown in Fig. 3 \ref{fig:LLM_for_KGQA}, DEKCOR \cite{xu2021fusing} concatenates the retrieved facts with questions and candidate answers as
\begin{equation}
    x = \texttt{[CLS]} \  q \  \texttt{[SEP]} \  \text{Related Facts} \  \texttt{[SEP]} \  a \  \texttt{[SEP]},
\end{equation}
where $a$ denotes candidate answers. Then, it feeds them into LLMs to predict answer scores. After utilizing LLMs to generate the representation of $x$ as QA context, DRLK \cite{zhang2022drlk} proposes a Dynamic Hierarchical Reasoner to capture the interactions between QA context and answers for answer prediction. Yan et al. \cite{yan2021large} propose a LLM-based KGQA framework consisting of two stages: (1) retrieve related facts from KGs and (2) generate answers based on the retrieved facts. The first stage is similar to the entity/relation extractors. Given a candidate answer entity $a$, it extracts a series of paths $p_1,\ldots,p_n$ from KGs. But the second stage is a LLM-based answer reasoner. It first verbalizes the paths by using the entity names and relation names in KGs. Then, it concatenates the question $q$ and all paths $p_1,\ldots,p_n$ to make an input sample as
\begin{equation}
    x = \texttt{[CLS]} \  q \  \texttt{[SEP]} \  p_1 \  \texttt{[SEP]} \  \cdots \  \texttt{[SEP]} \  p_n \  \texttt{[SEP]}.\label{eq:answer_reasoner}
\end{equation}
These paths are regarded as the related facts for the candidate answer $a$. Finally, it uses LLMs to predict whether the hypothesis: ``$a$ is the answer of $q$'' is supported by those facts, which is formulated as
\begin{align}
    e_\texttt{[CLS]} & = \text{LLM}(x),                                                        \\
    s                & = \sigma(\text{MLP}(e_\texttt{[CLS]})),\label{eq:answer_reasoner_score}
\end{align}
where it encodes $x$ using a LLM and feeds representation corresponding to $\texttt{[CLS]}$ token for binary classification, and $\sigma(\cdot)$ denotes the sigmoid function.

To better guide LLMs reason through KGs, OreoLM \cite{hu2022empowering} proposes a Knowledge Interaction Layer (KIL) which is inserted amid LLM layers. KIL interacts with a KG reasoning module, where it discovers different reasoning paths, and then the reasoning module can reason over the paths to generate answers. GreaseLM \cite{zhang2022greaselm} fuses the representations from LLMs and graph neural networks to effectively reason over KG facts and language context. UniKGQA \cite{jiang2023unikgqa} unifies the facts retrieval and reasoning into a unified framework. UniKGQA consists of two modules. The first module is a semantic matching module that uses a LLM to match questions with their corresponding relations semantically. The second module is a matching information propagation module, which propagates the matching information along directed edges on KGs for answer reasoning. Similarly, ReLMKG \cite{cao2022relmkg} performs joint reasoning on a large language model and the associated knowledge graph. The question and verbalized paths are encoded by the language model, and different layers of the language model produce outputs that guide a graph neural network to perform message passing. This process utilizes the explicit knowledge contained in the structured knowledge graph for reasoning purposes. StructGPT \cite{jiang2023structgpt} adopts a customized interface to allow large language models (e.g., ChatGPT) directly reasoning on KGs to perform multi-step question answering.


==> sections/applications.tex <==
\section{Applications}
\subsection{Search Engine}
\subsection{Conversational Agents}
\subsection{Recommendation}
